The Grothendieck-Teichm\"uller group of a finite group and $G$-dessins d'enfants

For each finite group G, we define the Grothendieck-Teichm\"uller group of G, denoted GT(G), and explore its properties. The theory of dessins d'enfants shows that the inverse limit of GT(G) as G varies can be identified with a group defined by Drinfeld and containing the absolute Galois group of the rational field. We give in particular an identification of GT(G), in the case when G is simple and non-abelian, with a certain very explicit group of permutations that can be analyzed easily. With the help of a computer, we obtain precise information for G= PSL(2, q) when q= 4, 7, 8, 9, 11, 13, 16, 17, 19, and we treat A7, PSL(3, 3) and M11. In the rest of the paper we give a conceptual explanation for the technique which we use in our calculations. It turns out that the classical action of the Grothendieck-Teichm\"uller group on dessins d'enfants can be refined to an action on equivariant dessins, which we define, and this elucidates much of the first part.

==> simple.tex <==
\section{Generalities}

\subsection{Definitions}


Suppose that~$\Gamma $ is a finite group, generated by two distinguished elements~$x$ and~$y$, and such that \begin{enumerate}
\item $\Gamma $ has an automorphism~$\theta $ such that~$\theta (x) = y$ and~$\theta (y) = x$,
\item $\Gamma$ has an automorphism~$\delta $ such that~$\delta (x)=z$ and~$\delta (y) = y$, where~$z$ is the element such that~$xyz=1$.
\end{enumerate}

In this situation we define~$A(\Gamma )$ to be the following subgroup of~$Out(\Gamma )$ : an element~$\phi \in Aut(\Gamma )$ represents an element of~$A(\Gamma )$, by definition, when \begin{enumerate}
\item $\phi(x)$ is conjugated to~$x^k$ for some~$k$ prime to the order of~$\Gamma $,
\item $\phi$ commutes with~$\theta $ and~$\delta $ in~$Out(\Gamma )$.
\end{enumerate}

(It follows that~$\phi(y)$ is conjugated to~$y^k$, and likewise for~$z$.)

Here is a way to produce examples of groups~$\Gamma $ with the above properties (in fact, the only examples we care about) : start with any finite group~$G$ with distinguished generators~$x$ and~$y$, and build~$\overline G$; recall that this is~$\langle x, y \rangle / N$ where~$N$ is the intersection of all the normal subgroups~$N_i$ such that~$\langle x, y \rangle /N_i \cong G$ (as groups, not as groups-with-distinguished-generators).

Finally, we define~$\gt(G) = A(\overline G)$, and call it the Grothendieck-Teichmüller group of~$G$. (In~\cite{pedro} this was denoted by~$\gt(N)$ where~$N$ is the normal subgroup above.)

How~$\gt(G)$ varies with~$G$ is a discussion which we postpone to the next subsection. For the time being, we take it for granted that it is possible to form the inverse limit
%
\[ \gt := \lim_G \gt(G) \, .   \]
%
In~\cite{pedro} we proved the motivating result that there is a monomorphism
%
\[ \gal \longrightarrow \gt \, .   \]
% 

{\em Project: compute~$\gt(G)$ on many examples, preferably coming in families.}

\begin{ex}
Here is the simplest example of such a family. Let~$C_n$ be cyclic of order~$n$; then~$\overline C_n = C_n \times C_n$. It follows easily that~$\gt(C_n)$ is comprised of the automorphisms~$x \mapsto x^k$, $y \mapsto y^k$ for~$k$ prime to~$n$, so~$\gt(C_n) \cong \left(\z/n\right)^\times $. Letting~$n$ vary, we obtain
%
\[ \lim_{C_n} \gt(C_n) \cong \widehat\z^\times \, ,  \]
% 
the group of units in the profinite completion of the ring~$\z$. (Again, we postpone to the next subsection an argument justifying {\em a priori} that the inverse limit of the groups~$\gt(C_n)$ makes sense.)


Projecting from~$\gt$ to~$\lim_{C_n} \gt(C_n)$, we see that there is a map~$\gt \to \hat \z^\times$, and so also a map
%
\[ \gal \longrightarrow \widehat\z^\times \, .  \]
%
The results in~\cite{pedro} show that it can be identified with the cyclotomic character (sending~$\lambda \in \gal$ to ``what it gives on the roots of unity''). This homomorphism is famous in number theory; it is known to be surjective, and the kernel is precisely the subgroup of commutators.

{\em Other families of groups will give generalizations of the cyclotomic character}, hopefully telling us something ``nonabelian'' about~$\gal$.


\end{ex}


We also define the subgroup~$A'(\Gamma )$ of~$A(\Gamma )$, comprised of those elements satisfying the condition above for~$k=1$. We put~$\gtz(G) = A'(\gb)$, and~$\gtz = \lim_G \gtz(G)$. The results of~\cite{pedro} show (using different notation) that~$\gtz$ is the kernel of the map~$\gt \to \hat\z^\times$. Moreover, there is an injective map
%
\[ \Gal( \qb / \q^{ab}) \longrightarrow \gtz \, .   \]
%

We can also offer the following elementary comments, all related to the question of whether an element~$\phi \in A(\Gamma )$ determines the integer~$k$ non-ambiguously. Suppose we have some homomorphism~$\Gamma \to \z/e$, for some integer~$e$, sending~$x$ to a generator of the cyclic group~$\z/e$ (a similar discussion applies to~$y$ or~$z$); for example if~$\Gamma = \gb$ it suffices to find such a homomorphism on~$G$ rather than~$\gb$. Then the elements~$x^k$ and~$x^\ell$ cannot be conjugated in~$\Gamma $ unless~$k=\ell$ modulo~$e$. There results a (well-defined!) map
%
\[ K_e \colon A(\Gamma ) \longrightarrow  \left(\z / e\right)^\times \, ,  \]
%
sending~$\phi$ to~$k$ modulo~$e$. Of course the kernel of~$K_e$ contains~$A'(\Gamma )$. Note that it may well be impossible to do better than~$e= 1$, for example when~$G$ is a non-abelian, simple group and~$\Gamma = \gb$.

Suppose nevertheless than we have a family of groups~$\Gamma_n$ and corresponding integers~$e_n$, together with the compatibilities allowing us to speak of the combined homomorphism
%
\[ K \colon \lim_{\Gamma_n} A(\Gamma_n) \longrightarrow \lim_n \left(\z /
e_n\right)^\times \, ; \]
%
assume further than any integer at all divides some~$e_n$, so that~$\lim_n \left(\z / e_n\right)^\times \cong \hat\z^\times$. Then it is elementary to check that the kernel of~$K$ is~$\lim_{\Gamma_n} A'(\Gamma_n)$.

%% We offer
%% the following comments. Let~$e$ be the exponent of the abelian
%% group~$\Gamma / [\Gamma , \Gamma ]$; this group is of the form~$\z/e
%% \times \z/e$ or possibly just~$\z/e$, given our assumptions on~$\Gamma
%% $. ({\footnotesize verified!}) Suppose given an element of~$\Gamma $
%% which is conjugated to~$x^k$ for some~$k$: then the integer~$k$ is
%% well-defined modulo~$e$ (or in other words~$x^k$ and~$x^\ell$ are not
%% conjugate in~$\Gamma $ unless~$k=\ell$ modulo~$e$). We obtain a
%% homomorphism
%% %
%% \[ A(\Gamma ) \longrightarrow \left(\z / e\right)^\times  \]
%% %
%% mapping~$\phi$ to~$k$, whose kernel we write~$A''(\Gamma )$. We
%% have~$A'(\Gamma ) \subset A''(\Gamma )$ with equality when the order
%% of~$x$ (or~$y$ or~$z$) in~$\Gamma $ is~$e$, rather than a multiple
%% of~$e$. 

%% In practice however, we will only find {\em some} integer~$f$ such
%% that there is an homomorphism~$\Gamma \to \z/f$ mapping, say, $x$ to a
%% generator ($y$ or~$z$ will do equally well). Then there is
%% map~$A(\Gamma ) \to \left(\z/f\right)^\times$ mapping~$\phi$ to~$k$,
%% and its kernel contains~$A'(\Gamma )$. Informally ``at least~$k$ is
%% well-defined modulo~$f$''. 

%% Let us write~$\gtz(G)$ for~$A'(\gb)$. We can construct a map~$\lim_G
%% \gt(G) \to \hat\z^\times$ by projecting to~$\lim_{C_n} \gt(C_n) \cong
%% \hat\z^\times$ (again, see the next subsection to see that this
%% inverse limit is well-defined). The resulting homomorphism essentially
%% sends~$\phi$ to~$k$, and its kernel is~$\lim_G \gtz(G)$.

%% One last comment is that there is an injective homomorphism 
%% %
%% \[ \gal^{ab} \longrightarrow \lim_G \gtz(G) \, ,  \]
%% %
%% motivating the definition.
 
\begin{rmk}
Whenever~$\Gamma = \gb$ for some group~$G$, then any homomorphism~$A(\Gamma ) \to \left(\z/e\right)^\times$ constructed as above is automatically surjective. The only (very indirect) argument we have is that whenever an element~$\phi$ of~$A(\Gamma )$ comes from an element of~$\lambda \in \gal$, then the integer~$k$ can be computed by considering the action of~$\lambda $ on the roots of unity in~$\qb$. Of course there exist elements~$\lambda $ with arbitrary prescribed action on those roots, and the claim follows. It would be interesting to have a direct proof.
\end{rmk}







%% A final remark. For any group~$G$ at all, let~$n$ be the order of~$x$
%% (or~$y$) in~$\overline G$; then there is a homormorphism 
%% %
%% \[ \gt(G) \longrightarrow \left(\z/n\right)^\times  \]
%% %
%% sending~$\phi$ to~$k$ (and~$\phi(x)$ is conjugated to~$x^k$). It is
%% surjective. Its kernel we write~$\gtz(G)$. 



\subsection{Functoriality}

When talking about the inverse limit~$\lim_G \gt(G)$, we mean to take into consideration all the maps of the form~$\gb \to \gb'$ mapping the canonical generators~$x, y$ of~$G$ to the canonical generators~$x', y'$ of~$G'$. Then we note:

\begin{lem}
Whenever there is a map~$\gb \to \gb'$ preserving the canonical generators, it is surjective and its kernel is characteristic in~$\gb$. Thus there is an induced map
%
\[ \gt(G) \longrightarrow \gt(G') \, .   \]
%
\end{lem}



Perhaps it is useful to give examples of such maps.

\begin{lem}
Let~$G$ and~$G'$ be finite groups, and fix a homomorphism~$\pi \colon G \to G'$. Suppose that whenever~$G'$ is generated by two elements~$a'$ and~$b'$, there exist elements~$a, b \in G$ generating~$G$ such that~$\pi(a) = a'$, ~$\pi(b)=b'$.

Then there is a homomorphism~$\gb \to \gb'$ mapping~$x$ to~$x'$ and~$y$ to~$y'$.
\end{lem}


\begin{ex}
We can at least deal with cyclic groups. Let~$G' = \z/n$ and~$G = \z/nm$, while the map~$\pi$ is induced by the identity of~$\z$. To see that the lemma applies, we may use the Chinese remainded theorem to reduce to the case when~$n$ and~$m$ are both powers of a prime~$p$, that is to the map~$\z/p^\beta \to \z/p^\alpha $ with~$\beta \ge \alpha $. If~$a'$ and~$b'$ together generate~$\z/p^\alpha $, we lift them to integers~$A$ and~$B$ and observe that~$A$ and~$B$ cannot be both divisible by~$p$. Hence one of them, say~$A$, is prime to~$p^\beta $, so that the images~$a$ and~$b$ of~$A$ and~$B$ in~$\z/p^\beta $ generate this group. They clearly map to~$a'$ and~$b'$.

It follows that there are maps~$\gt(C_{nm}) \to \gt(C_n)$, and it makes sense to talk about the inverse limit
%
\[ \lim_{C_n} \gt(C_n) \, ,  \]
%
as we have already done.
\end{ex}


%% \begin{ex}
%% The following situation will appear in the sequel: a finite group~$G$
%% with two generators~$s$ and~$t$ each of order~$N$, such that the
%% abelianization~$G' = G / [G, G] \cong \z/N$ is cyclic of order~$N$,
%% generated by the image of either~$s$ or~$t$. Let us show that the
%% first lemma applies. Indeed, supoose that~$a'$ and~$b'$ are integers
%% whose images generate~$\z/N$, and by Bézout, pick~$u$ and~$v$ such
%% that~$N$ divides~$ua' + vb'-1$. If we put~$a = s^{a'}$ and~$b =
%% s^{vb'-1} t$, we see that~$a^ub = s^{ua' + vb'-1} t = t $



%% Then the first lemma
%% clearly applies, resulting in a map~$\gt(G) \to \gt(\z/N) =
%% \left(\z/N\right)^\times$. 
%% \end{ex}





\subsection{$p$-groups}

\begin{prop}
When~$G$ is a~$p$-group, so is~$\gt(G)$.
\end{prop}

\begin{proof}
First note that~$\gb$ is itself a~$p$-group. Let~$\tilde A(\gb)$ denote the preimage of~$A(\gb)$ in~$Aut(\gb)$. If~$\tilde A(\gb)$ is not a~$p$-group, then it contains an element~$\phi$ whose order is a prime~$\ell \ne p$.

Consider the elementary abelian~$p$-group~$E =\gb / \Phi(\gb)$, where~$\Phi(\gb)$ is the Frattini subgroup of~$\gb$, generated by the images~$\bar x$ and~$\bar y$ of~$x$ and~$y$. The induced action of~$\phi$ on~$E$ sends~$\bar x$ to~$\bar x^k$, and likewise for~$\bar y$; so~$\phi^\ell = Id$ maps~$\bar x^k$ to~$\bar x^{k\ell} = x$, and because~$\ell \ne p$ we are led to conclude that~$p$ divides~$k$. As a result, the action of~$\phi$ on~$E$ is trivial.

It follows from~\cite{isaacs}, Corollary 3.29, that the action of~$\phi$ on~$\gb$ is trivial, violating the assumption that the order of~$\phi$ is~$\ell$. This contradiction shows that~$\tilde A(\gb)$ is a~$p$-group, and so also is~$A(\gb) = \gt(G)$.
\end{proof}


TO DO : insert result about the order of~$\gt(G)$ when~$G$ is a~$p$-group.




















\section{The dihedral groups}

To give an idea of the sort of computations to achieve, here we take the example of~$G= D_n$, the dihedral group of order~$2n$. (Below we explain that the result is not too useful, but at least we can perform the computation).


I will say very little about the proof, but still, let~$s$ and~$t$ be involutions generating~$D_{n}$, and let~$R= st$. The group~$\Gamma = \overline D_{n}$ is the subgroup of~$D_n \times D_n \times D_n$ generated by~$x=(s, R, s)$ and~$y = (t, t, R)$.

First is the case when~$n$ is odd. In this case I have proofs for all the facts stated now. The group~$\Gamma $ has order~$4n^3$, so it is of index~$2$ in~$D_n \times D_n \times D_n$, and thus it is normal. The element~$g=(t, 1, 1)$ is not in~$\Gamma $ and conjugation by~$g$ gives a candidate~$\phi \in Out(G)$. It turns out that~$\gtz(G)$ has just two elements, the identity and the class of~$\phi$.

To give a taste of the calculation, one establishes the following. We will find the orbits of~$C_G(y)$, the centralizer of~$y$, on~$x^G$, the conjugacy class of~$x$. Indeed if~$\phi$ is an automorphism of~$\Gamma $ representing an element of~$\gtz(G)$, then we can arrange to have~$\phi(y) = y$ and~$\phi(x) = x' \in x^G$, and two choices~$x'$ and~$x''$ give the same element in~$Out(\Gamma )$ if and only if they are in the same~$C_G(y)$-orbit.


There are $2n^2$ ways to pick an element~$(s', R', s'')$ conjugated to~$x=(s, R, s)$ in~$D_n^3$, since all the~$n$ involutions in~$D_n$ are conjugate (while the class of~$R$ is~$\{ R, R^{-1} \}$); however the centralizer of~$x$ in~$G$ is the subgroup generated by~$x$, of order~$2n$, so the order of the conjugacy class of~$x$ within~$G$ has size~$4n^3 / 2n = 2n^2$. So we have described all the conjugates.

The centralizer of~$y$ acts freely of the class of~$x$ (essentially because the centre of~$D_n$ is trivial), giving~$n$ orbits of size~$2n$. If~$x' = (s', R', s'')$ is conjugated to~$x$, write~$s'= sR^m$, then~$x'$ and~$y$ generate~$G$ if and only if~$m$ is prime to~$n$, leaving~$\varphi(n)$ choices for~$\phi$. One can see that they all give well-defined automorphisms (in fact, if~$x'$ and~$y'$ are two generators of~$\Gamma $, then there is automatically an automorphism taking~$x, y$ to~$x', y'$).

Finally, checking which of these commute with~$\delta $ imposes~$m=0$ or~$m=2$. These are the two final choices.

When~$n$ is even, I do not have proofs for the following facts, but they have been checked by computer for many values of~$n$. It turns out that if~$n= 2k$, then the order of~$\Gamma $ is~$4k^3$ (and not~$4n^3$). The group~$\gtz(G)$ is trivial when~$k$ is even, and has just two elements when~$k$ is odd.




In the end we see that~$\gtz(D_n)$ is trivial when~$n$ is divisible by~$4$. Sadly we conclude that
%
\[ \lim_n \gtz(D_n) = 1 \, .   \]
%


%% We have an exact sequence 
%% %
%% \[ 1 \longrightarrow \z/2 \longrightarrow \gt(D_n) \longrightarrow
%% \left(\z/(2n)\right)^\times \longrightarrow 1 \]
%% %
%% (well except when~$n$ is divisible by~$4$...), and so an exact sequence 
%% %
%% \[ 1 \longrightarrow \z/2 \longrightarrow \lim_n \gt(D_n)
%% \longrightarrow \widehat\z^\times \longrightarrow 1  \]
%% %
%% (or something close...). The cyclotomic character thus lifts to this
%% extension of~$\widehat\z^\times$, which seems exciting. However, since
%% an extension of a cyclic group by~$\z/2$ has to be abelian, we see
%% that~$\lim_n \gt(D_n)$ is abelian. It follows that the image of~$\gal$
%% within this group actually injects into~$\widehat\z^\times$ (the
%% kernel of the projection to this group being comprised of commutators,
%% as pointed out above). So we do not really get finer information
%% on~$\gal$. 

%% What is worse, I have tried to let the automorphism~$\phi$ above act
%% on dessins -- that is, on conjugacy classes of subgroups of~$\Gamma
%% $. It seems to always act trivially ! (And my computer has tried many,
%% many examples.)

%% Next in line are the generalized quaternion groups, which are
%% extensions of the dihedral groups, I guess... Other groups to look at
%% include the holomorphs~$C_n \rtimes Aut(C_n)$, and it seems possible
%% to say a lot about~$\gt(G)$ when~$G$ is simple (though in this case it
%% does not come within a family).




































\section{The case of simple groups}

In~\cite{gareth} one finds a proof of the following

\begin{lem}
Let~$G$ be a nonabelian, simple finite group. Then \begin{enumerate}
\item For any integer~$r$, the normal subgroups of~$G^r$ are those of the form~$\prod_I G_i$ for some~$I \subset \{ 1, \ldots, r \}$ (where~$G_i$ is the~$i$-th embedded copy of~$G$ in~$G^r$).

\item As a result, the maximal, proper normal subgroups of~$G^r$ are those of the form~$\prod_{i \ne j} G_i $ for some~$j$. Call it~$M_j$.

\item The group~$\gb$ is isomorphic to~$G^r$ where~$r$ is the number of orbits of pairs of generators~$(x,y)$ for~$G$ under~$Aut(G)$.
\end{enumerate}
\end{lem} 

In the rest of this section~$G$ will always be nonabelian and simple, as well as finite. Let us add :

\begin{lem} The automorphisms of~$G^r$ are as follows:
\begin{enumerate}
\item $Aut(G^r) \cong Aut(G) \wr S_r$.
\item $Out(G^r) \cong Out(G) \wr S_r$.
\end{enumerate}
\end{lem}

\begin{proof}
Considering the action on the~$M_j$'s, we obtain a map~$Aut(G^r) \to S_r$ which is clearly split surjective. Now suppose~$\phi$ is an automorphism of~$G^r$ preserving all the~$M_j$'s. By taking intersections, we see that~$\phi$ preserves all the normal subgroups of~$G^r$, including~$G_1$ and~$M_1 \cong G^{r-1}$, these two satisfying~$G_1 \times M_1 = G^r$. By induction, it is immediate that~$\phi$ is of the form~$\alpha_1 \times \cdots \times \alpha_r$. This proves (1).

An inner automorphism must preserve all the normal subgroups, so it is of the form just indicated, and so must be the direct product of inner automorphisms of each~$G_i$. This proves (2).
\end{proof}

We give a description of~$\gt(G)$ in the special case when~$Out(G)$ has order~$2$. The case when~$Out(G)$ is trivial will be an obvious simplification of the argument which follows (we comment on this below), while the case when~$Out(G)$ is abelian would just require more notation and care. We point out that the nonabelian finite simple groups~$G$ such that~$Out(G)$ has order~$1$ or~$2$ include the alternating groups, almost all Chevalley groups over~$\f_p$ where~$p$ is prime (but not a prime power), and all 26 sporadic groups. I am not sure if~$Out(G)$ can be nonabelian.


Let~$\pairs$ denote the set of pairs of elements~$(x, y)$ generating~$G$. The group~$Aut(G)$ acts on~$\pairs$, and the set~$\pairs / Aut(G)$ of orbits has cardinality~$r$. However it will be technically more convenient to work with~$\pc$, the set of orbits under the sole action of the inner automorphisms. We see that~$Out(G)$ acts freely on~$\pc$, and~$\pc / Out(G) = \pairs / Aut(G)$. With our hypothesis, the set~$\pc$ has cardinality~$2r$.

Let~$\alpha \in Aut(G)$ represent a generator for~$Out(G)$. We fix a numbering of the elements in~$\pairs/Aut(G)$, so that we may conveniently identify this set with~$\{ 1, \ldots, r \}$. Likewise, we may identify~$\pc$ with~$\{ 1, \ldots, 2r \}$; in fact we arrange things as follows: the number~$i$ with~$1 \le i \le r$ corresponds to a class~$C \in \pairs/Aut(G)$ which splits as two classes numbered~$i$ and~$r+i$ in~$\pc$. The permutation~$(1, r+1)(2, r+2), \ldots, (r, 2r)$ induced by~$\alpha $ will be written~$\pi_\alpha $.

Recalling that~$\gb = G^r$ as above, we introduce the embedding
%
\[ G^r \longrightarrow G^{2r} = G^r \times G^r  \]
%
%
\[ g \mapsto (g, g^\alpha ) \, .   \]
%
The image of this embedding we write~$G^{r, r}$.

\begin{rmk}
The automorphism~$\alpha \times \alpha $ of~$G^{2r}$ preserves the subgroup~$G^{r, r}$. Suppose that~$\alpha^2$ is the identity (which is stronger than our hypothesis, according to which~$\alpha^2$ is inner). Then (the automorphism induced by) the permutation~$\pi_\alpha $ also preserves~$G^{r, r} $ and agrees with~$\alpha \times \alpha $ on this subgroup. In general however, we can only state that we can compose~$\pi_\alpha $ with an inner automorphism of~$G^{2r}$ in order for~$G^{r, r}$ to be preserved. Such subtleties creep up a lot in what follows, making the arguments a little trickier than they seem.
\end{rmk}

Recall the descriptions of~$Aut(G^r)$ and~$Aut(G^{2r})$ in the above lemma. They both contain a canonical copy of a symmetric group, and we shall speak of {\em permutation automorphisms} of~$G^r$ and~$G^{2r}$, the meaning of which should be clear; and we shall say that~$\phi \in Aut(G^{2r})$ is an {\em almost-permutation automorphism} when it is the composition of a permutation automorphism and an inner automorphism. Almost-permutation automorphisms form a subgroup~$\almost(G^{2r})$ of~$Aut(G^{2r})$, and we shall write~$\almost(G^{2r}, G^{r,r})$ for those almost-permutation automorphisms which preserve the subgroup~$G^{r, r}$.

We have natural maps
%
\[ p \colon \almost(G^{2r}, G^{r, r}) \longrightarrow S_{2r}  \]
%
and
%
\[ q \colon   \almost(G^{2r}, G^{r, r}) \longrightarrow Out(G^{r, r})
= Out(G^{r}) \, .  \]
%


\begin{prop}
Let~$C$ be the centralizer of~$\pi_\alpha $ in~$S_{2r}$. Then there is a commutative diagram
%
\[ \xymatrix{ & \almost(G^{2r}, G^{r, r}) \ar[ld]_q \ar[rd]^p & \\ 
Out(G^r) \ar[rr]^\iota & & C } \]
%
Both~$p$ and~$q$ are surjective, and~$\iota $ is an isomorphism.
\end{prop}

In the sequel it will prove useful, not only to have an isomorphism between the group~$Out(G^r)$ and the centralizer of~$\pi_\alpha $, but also to be able to work with the maps~$p$ and~$q$ which are so explicit and simple.

\begin{proof}
{\em Step 1.} We prove that the map~$p$ actually takes its values in~$C$. Recall the maximal, normal subgroups~$M_1, \ldots, M_{2r}$ of~$G^{2r}$. The maximal, normal subgroups of~$G^{r, r}$ are of the form~$M_i \cap G^{r, r}$, and the equality~$M_i \cap G^{r, r} = M_j \cap G^{r, r}$ happens if and only if~$|i - j|=r$ or~$0$, that is, if and only if~$i$ and~$j$ are exchanged by~$\pi_\alpha $.

Now if~$\phi $ preserves~$G^{r, r}$, writing~$\sigma = p(\phi)$ we have~$\phi (M_i \cap G^{r, r}) = M_{\sigma(i)} \cap G^{r, r}$ and this must be equal to~$M_{\sigma (\pi_\alpha (i))} \cap G^{r, r}$. It follows that~$\{ \sigma (i), \sigma (\pi_\alpha (i)) \}$ is stable under~$\pi_\alpha $, and if we keep in mind that~$\pi_\alpha $ is an involution without fixed point, we see that~$\sigma $ and~$\pi_\alpha $ commute.

{\em Step 2.} We prove that~$p$ is surjective. This follows from the description of the centralizer~$C= C_{S_{2r}}(\pi_\alpha )$ under consideration. Indeed, it is of the form~$C_2 \wr S_r = C_2^r \rtimes S_r$, where the elementary abelian subgroup~$C_2^r$ is generated by the involutions~$(i, r+i)$, and the map~$C \to S_r$ is obtained by looking at the induced action on the set of orbits of~$\pi_\alpha $. This is abstractly isomorphic to~$Out(G^r)$, of course. Concretely if~$\sigma \in C$, the corresponding element~$\sigma ' \in S_r$ can be immediately lifted to a permutation automorphism of~$G^{2r}$ preserving~$G^{r, r}$ (simply extend~$\sigma '$ to~$\{ 1, \ldots, 2r \}$ by requiring~$\sigma '(r+i) = r + \sigma '(i)$). On the other hand the permutation automorphism given by~$(i, r+i)$ does not preserve~$G^{r, r}$, but the fact that~$\alpha^2$ is inner means that we can compose it with a conjugation in~$G^{2r}$ and obtain an automorphism which does preserve~$G^{r, r}$ (this is similar to the issue raised in the Remark above).

{\em Step 3.} We prove that~$p$ factors through~$\ker q$. So let~$\phi \in \almost(G^{2r}, G^{r, r})$, let~$\sigma = p(\phi)$, and assume that~$q(\phi) = 1$, that is, $\phi$ is inner when restricted to~$G^{r, r}$. We want to show that~$\sigma = 1$.

The fact that~$q(\phi)= 1$ implies that~$\phi$ preserves the maximal, normal subgroups of~$G^{r, r}$, and from this we see that
%
\[ \sigma = \prod_{\textnormal{some}~i} (i, r+i) \, .   \]
%
We must show that the product is in fact empty. For simplicity of notation, say that~$\sigma $ contains~$(1, r+1)$. The effect of~$\phi$ on
%
\[ (x_1, \ldots, x_r, x_1^\alpha , \ldots, x_r^\alpha ) \in G^{r, r}
\, , \]
%
focusing attention on the first coordinate, is~$x_1 \mapsto c^{-1} x_1^\alpha c$ for some~$c \in G$. Since~$\phi$ is assumed to be inner on~$G^{r, r}$, we conclude absurdly that~$\alpha $ is inner. This shows that~$\sigma $ contains no~$(i, r+i)$, so~$\sigma = 1$.

{\em Conclusion.} There must be a map~$\iota $ such that~$p = \iota \circ q$, and it is automatically surjective just like~$p$ is. Since~$Out(G)$ and~$C$ both have order~$2^r r!$, we deduce that~$\iota $ is in fact an isomorphism.
\end{proof}





%% \begin{lem}
%% \begin{enumerate}
%% \item Let~$\tilde \sigma \in Aut(G^{2r})$ be an almost-permutation
%%   automorphism. If~$\tilde \sigma $ preserves~$G^{r, r}$, then~$\sigma $
%%   commutes with~$\pi_\alpha $ in~$S_{2r}$.

%% \item If the permutation~$\sigma $ commutes with~$\pi_\alpha $
%%   in~$S_{2r}$, then we can lift it to an almost-permutation
%%   automorphism~$\tilde \sigma $ of~$G^{2r}$ which preserves~$G^{r,
%%     r}$.

%% \item There is an injective map~$Out(G^r) \to S_{2r}$, written~$\phi
%%   \mapsto \sigma_\phi$, which identifies~$Out(G^r)$ with the centralizer
%%   of~$\pi_\alpha $ in~$S_{2r}$. Moreover, this identification is
%%   compatible with the above lifts in the following sense, where we
%%   have identified~$Out(G^r)$ and~$Out(G^{r, r})$: \begin{enumerate}
%% \item if~$\tilde \sigma $ is an almost-permutation automorphism
%%   preserving~$G^{r, r}$, as in (1), and if we write~$\phi$ for the
%%   induced element of~$Out(G^r)$, then~$\sigma_\phi = \sigma $ ;
%% \item if~$\sigma_\phi$ is lifted to an almost-permutation
%%   automorphism~$\tilde \sigma_\phi$ of~$G^{2r}$ preserving~$G^{r, r}$,
%%   as in (2), then~$\tilde \sigma_\phi$ agrees with~$\phi$
%%   in~$Out(G^r)$. 
%% \end{enumerate}
%% \end{enumerate}
%% \end{lem}

%% The proof will show that the third point follows from the first
%% two. More importantly, it will define the particular identification
%% which we use in (3) and in the sequel.

%% \begin{proof}
%% (1) Recall the maximal, normal subgroups~$M_1, \ldots, M_{2r}$
%%   of~$G^{2r}$. The maximal, normal subgroups of~$G^{r, r}$ are of the
%%   form~$M_i \cap G^{r, r}$, and the equality~$M_i \cap G^{r, r} = M_j
%%   \cap G^{r, r}$ happens if and only if~$|i - j|=r$ or~$0$, that is,
%%   if and only if~$i$ and~$j$ are exchanged by~$\pi_\alpha $.

%% Now if~$\sigma $ preserves~$G^{r, r}$, we have~$\sigma (M_i \cap G^{r,
%%   r}) = M_{\sigma(i)} \cap G^{r, r}$ and this must be equal
%% to~$M_{\sigma (\pi_\alpha (i))} \cap G^{r, r}$. It follows that~$\{
%% \sigma (i), \sigma (\pi_\alpha (i)) \}$ is stable under~$\pi_\alpha
%% $, and if we keep in mind that~$\pi_\alpha $ is an involution without
%% fixed point, we see that~$\sigma $ and~$\pi_\alpha $ commute.

%% (2) follows from the description of the centralizer~$C=
%% C_{S_{2r}}(\pi_\alpha )$ under consideration. Indeed, it is of the
%% form~$C_2 \wr S_r = C_2^r \rtimes S_r$, where the elementary abelian
%% subgroup~$C_2^r$ is generated by the involutions~$(i, r+i)$, and the
%% map~$C \to S_r$ is obtained by looking at the induced action on the
%% set of orbits of~$\pi_\alpha $. This is abstractly isomorphic
%% to~$Out(G^r)$, of course. Concretely if~$\sigma \in C$, the
%% corresponding element~$\sigma ' \in S_r$ can be immediately lifted to
%% a permutation automorphism of~$G^{2r}$ preserving~$G^{r, r}$ (simply
%% extend~$\sigma '$ to~$\{ 1, \ldots, 2r \}$ by requiring~$\sigma '(r+i)
%% = r + \sigma '(i)$). On the other hand the permutation automorphism
%% given by~$(i, r+i)$ does not preserve~$G^{r, r}$, but the fact
%% that~$\alpha^2$ is inner means that we can compose it with a
%% conjugation in~$G^{2r}$ and obtain an automorphism which does
%% preserve~$G^{r, r}$ (this is similar to the issue raised in the Remark
%% above).
%% \end{proof}

We are now ready to describe the subgroup~$\gt(G) \subset Out(G^r)$ as a subgroup of~$C$. We recall the definitions of the automorphisms~$\theta $ and~$\delta $ of~$G^r$, which involve some arbitrary choices; this arbitrariness disappears in~$Out(G^r)$ and so also in~$C$, and the Proposition will help us prove that.

For each class~$P_i \in \pairs/Aut(G)$ (with~$1\le i \le r$) we pick a representative~$(x_i, y_i)$ arbitrarily. Now put
%
\[ x = (x_1, \ldots, x_r) ~\textnormal{and}~ y=(y_1, \ldots, y_r) \,
.  \]
%
The elements~$x$ and~$y$ generate~$\gb = G^r$, and~$\theta $ is defined to be the automorphism satisfying~$\theta (x) = y$, $\theta (y) = x$. We construct now an element~$\tilde \theta \in \almost(G^{2r}, G^{r, r})$ such that~$q(\tilde \theta ) = \theta $ in~$Out(G^r)$, and such that~$\sigma = p(\tilde \theta )$ can be readily computed. It will follow that~$\sigma = \iota (\theta )$.

Finding~$\tilde \theta $ is easy (in principle -- in practice a computer is indispensable). First we move to~$G^{r, r}$ where we consider
%
\[ x' = (x_1, \ldots x_r, x_1^\alpha , \ldots, x_r^\alpha )
~\textnormal{and}~ y' = (y_1, \ldots, y_r, y_1^\alpha, \ldots, y_r^\alpha) \, , \]
%
and we will allow ourselves to write~$x_{r+i}$ instead of~$x_i^\alpha $. Let the classes in~$\pc$ be~$P_1^c, \ldots P_{2r}^c$. For each index~$i$ between~$1$ and~$2r$, the pair~$(y_i, x_i)$ generates~$G$ just like~$(x_i, y_i)$ does, so there must be a~$\tau (i)$ such that~$(y_i, x_i) \in P_{\tau (i)}^c$. This defines~$\tau \in S_{2r}$ and a permutation automorphism denoted by the same letter, and we let~$\sigma = \tau^{-1}$. Noting that~$\sigma (x_1, x_2, \ldots ) = (x_{\tau(1)}, x_{\tau (2)}, \ldots )$, we see that we can compose~$\sigma $ with an inner automorphism, obtaining~$\tilde \theta$ such that~$p(\tilde \theta) = \sigma $, in such a way that~$\tilde \theta(x') = y'$ and~$\tilde \theta(y') = x'$. (It is crucial, in order for these two equations to hold simultaneously, to keep in mind that~$(y_i, x_i)$ can be conjugated {\em as a pair} into~$(x_{\tau (i)}, y_{\tau (i)})$ by a single element of~$G$.)

In particular, $\tilde \theta$ must preserve~$G^{r, r}$ which is generated by~$x'$ and~$y'$, so~$\tilde \theta \in \almost(G^{2r}, G^{r, r})$ and clearly~$q(\tilde \theta) = \theta $, as required.

The elements of~$\gt(G)$ are required to commute with~$\theta $ in~$Out(G^r)$, and now this can be translated into the commutation with~$\sigma $ (or~$\tau $), when things are seen in~$C$ via~$\iota $.


We proceed similarly with~$\delta $, namely: the operation~$(x_i, y_i) \mapsto (y_i^{-1} x_i^{-1}, y_i)$ gives a permutation of the elements of~$\pc$, say~$\tau '$. The condition involving~$\delta $ is commutation with~$\tau '$ (or its inverse~$\sigma '$).

We have already identified the elements of~$\gt(G)$ as permutations in~$S_{2r}$ centralizing the subgroup generated by~$\sigma , \sigma ', \pi_\alpha $.


\begin{lem}
The subgroup generated by~$\sigma$ and~$\sigma '$ is a quotient of~$S_3$. The permutation~$\pi_\alpha $ commutes with both~$\sigma $ and~$\sigma '$, so that the subgroup generated by~$\sigma , \sigma '$ and~$\pi_\alpha $ is a quotient of~$S_3 \times C_2$.
\end{lem}

(To be inserted.)

To complete the description of the elements~$f \in \gtz(G)$, we must finally examine the condition that~$f(x)$ be conjugated to~$x$, and likewise that~$f(y)$ be conjugated to~$y$. (Of course if one of these holds, and~$f$ commutes with~$\delta $, the second condition also holds, though we shall not exploit this.)

The group~$G \times G$ acts on~$\pairs$ by conjugation. The orbits of~$G \times G$ break up into the disjoint union of orbits of the diagonal subgroup~$G$ ; put differently, we can group the elements of~$\pc$ into blocks (the union of the $G$-orbits in one block being a~$G\times G$-orbit). This affords a partition of~$\{ 1, \ldots, 2r \}$ and a corresponding Young subgroup~$Y$ of~$S_{2r}$.

Given~$f \in Out(G^r)$ and picking an element~$\phi \in \almost(G^{2r}, G^{r, r})$ inducing~$f$, it is readily seen that the conditions above on~$f$ translate into the requirement that the permutation~$\sigma = p(\phi)$ belong to the subgroup~$Y$.



\begin{thm}
Let~$G$ be a simple, nonabelian finite group. Let~$\pairs$ be the set of pairs of generators of~$G$, and let~$\pc$ be the set of orbits under inner automorphisms. Finally, let~$\alpha $ be a generator of~$Out(G)$, which is assumed to have order~$2$.

Write~$\pi_\alpha $ for the permutation of~$\pc$ induced by~$\alpha $; let~$Y$ be the Young subgroup of~$S(\pc)$ corresponding to the partition of~$\pc$ into elements belonging to the same~$G \times G$-orbit ; let~$\sigma $ be the permutation of~$\pc$ given by the operation~$(x, y) \mapsto (y, x)$ ; let~$\sigma '$ be the permutation of~$\pc$ given by~$(x, y) \mapsto (y^{-1} x^{-1}, y)$; and finally let~$C$ be the centralizer of~$\langle \sigma, \sigma ', \pi_\alpha \rangle$ in~$S(\pc)$.

Then the group~$\gtz(G)$ can be identified with the subgroup~$Y \cap C$ of~$S(\pc)$. Moreover~$\langle \sigma, \sigma ', \pi_\alpha \rangle$ is a quotient of~$S_3 \times C_2$.
\end{thm}

This Theorem severely restricts the isomorphism type of~$\gt(G)$ in this case. Briefly, examining the~$S_3 \times C_2$-sets, one sees that their automorphism groups are products of~$C_2$'s and~$S_3$'s; it follows that the centralizer~$C$ has a normal subgroup~$N$ which is also a product of groups of this type, and~$C/N$ is a product of symmetric groups. The same can be said of the intersection~$Y \cap C$. In particular

\begin{coro}
Under the hypotheses of the Theorem, the only possible simple factors of~$\gtz(G)$ are~$C_2$, $C_3$ and~$A_n$.
\end{coro}

\begin{ex}
Take~$G = PSL_3(\f_2)$, a simple group of order~$168$ with~$Out(G) = C_2$. The following information is obtained with GAP.

There are~$114$ elements in~$\pc$; in the following some arbitrary numbering is used for them. Looking at the action of~$G \times G$ we obtain the following partition of~$\{ 1, \ldots, 114 \}$ :
%
\begin{multline*}
\{ 1, 10, 27, 28, 96, 106 \}, \{ 2, 11, 52, 57, 82, 86 \}, \{ 3, 12 \}, \{ 62, 63 \}, \{ 107, 109 \}\\ \{ 4, 13, 29, 49, 51, 54, 56, 70, 101, 102 \}, \{ 5, 6, 31, 32, 71, 72 \}, \{ 7, 34, 75 \}, \{ 8, 84, 97 \}, \\\{ 9, 36, 53, 73, 83, 85 \}, \{ 14, 16, 38, 60, 91, 114 \}, \{ 15, 61, 76 \}, \{ 17, 98, 110 \},\\ \{ 18, 40, 58, 59, 78, 99 \}, \{ 19, 21 \}, \{ 20, 41, 43 \}, \{ 22, 42, 64 \}, \{ 39, 77, 90 \},\\\{ 23, 25, 44, 48, 67, 79, 87, 103, 108, 111 \}, \{ 24, 45, 68, 94, 105, 112 \}, \{ 33, 35, 74 \},\\ \{ 26, 46, 69, 89, 93, 104 \}, \{ 30, 37, 50, 55, 100, 113 \}, \{ 47, 65, 66, 80, 81, 88, 92, 95 \}.
\end{multline*}
%
There are 4 of size 2; 8 of size 3; 9 of size 6; one of size 8 and two of size 10. Thus~$Y \cong C_2^4 \times S_3^8 \times S_6^9 \times S_8 \times S_{10}^2$.

Then we compute \begin{itemize}


\item the permutation~$\pi_\alpha $ : (1,11) (2,10) (3,12) (4,101) (5,16) (6,14) (7,15) (8,17) (9,18) (13,102) (19,21) (20, 22) (23,48) (24,26) (25,103) (27,52) (28,57) (29,70) (30,100) (31,60) (32,38) (33, 77) (34,61) (35,39) (36,59) (37,113) (40,85) (41,42) (43,64) (44,87) (45,104) (46, 94) (47,88) (49,56) (50,55) (51,54) (53,58) (62,63) (65,80) (66,95) (67,111) (68, 93) (69,105) (71,114) (72,91) (73,78) (74,90) (75,76) (79,108) (81,92) (82,96) (83, 99) (84,110) (86,106) (89,112) (97,98) (107,109).

\item the permutation~$\sigma $ induced by~$\theta $ : (1,5) (2,14) (3,19) (4,23) (6,10) (7,15) (8,20) (9,24) (11,16) (12,21) (13,25) (17, 22) (18,26) (27,31) (28,72) (29,67) (30,100) (32,96) (34,61) (36,68) (38,82) (40, 69) (41,97) (42,98) (43,84) (44,49) (45,53) (46,99) (47,88) (48,101) (50,55) (51, 79) (52,60) (54,108) (56,87) (57,91) (58,104) (59,93) (62,107) (63,109) (64,110) (66, 95) (70,111) (71,106) (73,112) (75,76) (78,89) (81,92) (83,94) (85,105) (86,114) (102, 103).

\item the permutation~$\sigma '$ induced by~$\delta $ : (2,3) (4,106) (5,35) (6,8) (7,85) (10,12) (13,100) (14,17) (15,40) (16,39) (19,22) (20,21) (23,68) (24,65) (25,103) (26,80) (27,52) (28,70) (29,57) (30,102) (31,75) (34, 73) (36,71) (37,96) (41,63) (42,62) (44,87) (45,111) (46,107) (47,88) (48,93) (49, 55) (50,56) (51,54) (53,72) (58,91) (59,114) (60,76) (61,78) (66,108) (67,104) (69, 105) (74,84) (79,95) (81,92) (82,113) (83,97) (86,101) (89,112) (90,110) (94,109) (98, 99).

\end{itemize}

We can then ask GAP to compute~$\gtz(G)$ as the intersection of~$Y$ and the centralizer of the three permutations above. We find that~$\gtz(G)$ has order 512; its centre~$Z$ is elementary abelian of order~$32$; and~$\gtz(G)/Z$ is elementary abelian of order~$16$.

\end{ex}





















\section{Groups related to~$B_3$}

\subsection{The groups}

We start with the braid group~$B_3 = \langle \sigma_1, \sigma_2 : \sigma_1 \sigma_2 \sigma_1 = \sigma_2 \sigma_1 \sigma_2 \rangle$. There is a natural map~$B_3 \to S_3$ whose kernel is usually written~$P_3$ (the ``pure braid group''). The abelianization~$P_3 / [P_3, P_3]$ is isomorphic to~$\z^3$, endowed with the natural permutation action of~$S_3$.

Our first group of interest is~$G= B_3 / [P_3, P_3]$, which fits in an exact sequence
%
\[ 0 \longrightarrow \z^3 \longrightarrow G \longrightarrow S_3
\longrightarrow 0 \, .  \]
%

\begin{lem}
\begin{enumerate}
\item $G$ admits the presentation~$\langle s, t : sts= tst, [s^2, t^2] = 1 \rangle$.
\item The abelianization~$G/[G, G]$ is isomorphic to~$\z$, and the corresponding map~$G \to \z$ sends both~$s$ and~$t$ to~$1$.
\end{enumerate}
\end{lem}

\begin{lem}
There are just two exact sequences of the form
%
\[ 0 \longrightarrow \z^3 \longrightarrow H \longrightarrow S_3
\longrightarrow 0 \, , \]
%
where the action of~$S_3$ on~$\z^3$ is the natural permutation action. Either~$H = \z^3 \rtimes S_3$ when the extension is split, or~$H \cong G$ otherwise.
\end{lem}

\begin{proof}
As an~$S_3$-module, $\z^3$ can be seen as induced from the trivial~$C_2$-module, viewing~$C_2$ as a subgroup of~$S_3$ by picking any element of order~$2$. By Shapiro's lemma we have
%
\[ H^2(S_3, \z^3) \cong H^2(C_2, \z) \cong \z/2 \, .   \]
%
The statement about the number of extension follows. So will the rest of the lemma, if we can only prove that~$G$ is not a semi-direct product~$\z^3 \rtimes S_3$.

Indeed, if it were, it would possess an element~$x$ of order~$2$, mapping to an element of order~$2$ in~$S_3$. The image of~$x$ in~$\z$ via the abelianization map must be trivial, so~$x$ is in the commutator subgroup~$[G, G]$. However the commutator subgroup~$[S_3, S_3]$ has order~$3$ and cannot contain elements of order~$2$.
\end{proof}

Next we define a group~$G_n$ by reducing mod~$n$ the elements of~$\z^3 \subset G$. Thus there is an exact sequence
%
\[ 0 \longrightarrow \left(\z/n\right)^3 \longrightarrow G_n
\longrightarrow S_3 \longrightarrow 0 \, .  \]
%
(For example one can show that~$G_2 \cong SL(2, \z/4)$.) We propose to compute~$\gt(G_n)$. Let us first explain why these examples seem interesting. We shall see that when~$n$ divides~$m$, there is a natural map~$\gt(G_m) \to \gt(G_n)$, so we may form the inverse limit~$\lim_n \gt(G_n)$. The abelianization of~$G_n$ is~$\z/2n$, so there is a map~$\gt(G_n) \to \left(\z/2n\right)^\times$, and thus a map
%
\[ \lim_n \gt(G_n) \longrightarrow \widehat{\z}^\times \, ,  \]
%
as explained in the first section. The kernel of this map is clearly~$\lim_n \gtz(G_n)$. We obtain a lift of the cyclotomic character
%
\[ \gal \longrightarrow \lim_n \gt(G_n) \longrightarrow
\widehat{\z}^\times \, , \]
%
and to make it explicit we need to compute~$\gtz(G_n)$.





\subsection{Maps between the~$G_n$'s}

Our aim is to prove that there are maps~$\gb_m \to \gb_n$ when~$n$ divides~$m$, and the strategy is to prove that there is actually a canonical map~$\gb \to \gb_n$. Unfortunately we cannot quite prove this, and we are reduced to using an auxiliary group~$\widetilde G$, and to restrict attention to~$n$ prime to~$6 = |S_3|$.


We need a series of lemmas about~$\z[S_3]$-modules. We write~$A$ for~$\z^3$ with the natural action of~$S_3$. We denote the trivial module~$\z$ by~$T$; for example this module sits inside~$A$ as~$\langle a \rangle$, where~$a = (1, 1, 1)$. The submodule~$Z= \{ (x, y, z) : x + y + z = 0 \}$ of~$A$ will be important, as well as the quotient~$Q= A / \langle a \rangle $.

We mention that~$Z \cap \langle a \rangle = \{ 0 \}$, but the direct sum~$\langle a \rangle \oplus Z$ is not the whole of~$A$: rather, it consists of all elements~$(x, y, z)$ such that~$x+y+z$ is divisible by~$3$.

We write~$e_1, e_2, e_3$ for the canonical basis of~$A$, so that~$a= e_1 + e_2 + e_3$. The module~$Z$ is generated by~$e_1 - e_2$ and~$e_1 - e_3$, and~$Q$ is generated by the images of~$e_1$ and~$e_2$ which we usually write with the same letter, or~$\bar e_1, \bar e_2$ for emphasis. The image~$\bar Z$ of~$Z$ inside~$Q$ is (isomorphic to~$Z$ and) generated by~$e_1 - e_2$ and~$3 e_2$, which makes it clear that it has index~$3$ in~$Q$.

\begin{lem} \label{lem-submods-of-Q}
A sub-$S_3$-module of~$Q$ of rank~$2$ is either of the form~$kQ$ or~$k \bar Z$, for some~$k \ge 1$.
\end{lem}

\begin{proof}
Let~$R$ be such a module. The group~$Q/R$ is finite, generated by the images of~$e_1$ and~$e_2$, and these must have the same order in~$Q/R$, say~$\lambda $, by symmetry. So~$Q/R$ is a quotient of~$\z/\lambda \times \z/\lambda $.

Suppose there is a relation of the form~$a e_1 = be_2$ in~$Q/R$. Applying the permutation~$(1, 2)$ and adding the relations, we get~$a e_3 = b e_3$, where~$e_3 = -e_2 - e_1$. Applying~$(1, 3)$ we get~$ae_1 = be_1$ so~$\lambda $ divides~$b-a$. We may as well take~$a$ and~$b$ between~$0$ and~$\lambda $, and this forces~$a=b$.

So all the relations must be of the form~$a(e_1 - e_2) = 0$. We conclude that~$R$ is generated by~$\lambda e_1$, $\lambda e_2$ and~$a(e_1 - e_2)$ for some~$a$.

If~$k= gcd(a, \lambda )$, we see that~$R = kR'$ for some module~$R'$, so we only need to study the case~$k=1$. It follows at once that~$e_1 - e_2 \in R$, and this module is generated by~$\lambda e_1, \lambda e_2$ and~$e_1 - e_2$.

Applying~$(2, 3)$ to the relation~$ae_1 = be_2$ in~$Q/R$ gives~$(a+b)e_1 = -b e_2$, and the argument aboves shows that~$\lambda $ divides~$a+2b$, so in the end~$\lambda $ also divides~$3a$. Since we are assuming that~$gcd(a, \lambda )= 1$, we see that~$\lambda = 1$ or~$3$. If~$\lambda = 1$ then~$R = Q$, whereas if~$\lambda = 3$ then~$R = \bar Z$.
\end{proof}

\begin{lem}
Let~$n$ be an integer prime to~$3$.

\begin{enumerate}
\item The module~$A/n$ is isomorphic to~$T/n \oplus Z/n$.

\item The modules~$Z/n$ and~$Q/n$ are isomorphic.
\end{enumerate}
\end{lem}

\begin{proof}
(1) If~$Z'$ denotes the submodule of~$A/n$ of all those~$(x, y, z)$ such that~$x+y+z = 0 \in \z/n$, then the same elementary computation which works over~$\z$ shows that~$Z'$ is generated by~$e_1 - e_2$ and~$e_1 - e_3$ (in obvious notation). It follows that~$Z' \cong Z/n$.

For any~$v= (x, y, z) \in A/n$, let~$\ell = \frac{x+y+z} {3} \in \z/n$. Writing~$v = (v - \ell a) + \ell a$, we see that~$\langle a \rangle + Z' = A/n$; an element in the intersection of~$\langle a \rangle$ and~$Z'$ is of the form~$(k, k, k)$ with~$3k= 0 \in \z/n$, whence~$k=0$ and~$A/n = \langle a \rangle \oplus Z'$.

(2) We define two elements~$\varepsilon_1$ and~$\varepsilon_2$ of~$Z/n$ by~$\varepsilon_1 = -2e_1 + e_2 + e_3$ and~$\varepsilon_2 = e_1 - 2e_2 + e_3$. Then~$(1, 2)$ exchanges~$\varepsilon_1$ and~$\varepsilon_2$, while~$(2, 3)$ fixes~$\varepsilon_1$ and maps~$\varepsilon_2 $ to~$-\varepsilon_1 - \varepsilon_2$. So~$\langle \varepsilon_1, \varepsilon_2 \rangle$ is isomorphic to~$Q/n$. However~$\langle \varepsilon_1, \varepsilon_2 \rangle$ is all of~$Z/n$, for~$e_1 - e_2 = \frac{1} {3} (\varepsilon_1 - \varepsilon_2)$.
\end{proof}


\begin{lem}
Let~$M$ be a sub-$S_3$-module of~$A$ of rank~$3$, and let~$n$ be an integer prime to~$6$. Then
%
\[ M/n \cong A/n \, .   \]
%
\end{lem}

This actually holds under the sole assumption that~$n$ be prime to~$3$, but we will not prove this here.

\begin{proof}
The intersection~$M \cap \langle a \rangle$ is of the form~$\langle m \rangle$ for~$m = d a$ with~$d \in \z$. Let~$\bar M$ be the image of~$M$ in~$Q=A/\langle a \rangle$. Pick elements~$\varepsilon_1, \varepsilon_2 \in M$ mapping to generators of~$\bar M$ and put~$L= \langle \varepsilon_1, \varepsilon_2 \rangle$. The elements~$m, \varepsilon_1, \varepsilon_2$ generate~$M\cong \z^3$, so they form a basis for this module, and in particular~$M = \langle m \rangle \oplus L$.

Note that~$L$ is not an~$S_3$-module, in general. However, we also have~$M/n = \langle m \rangle /n \oplus L/n$, and in~$M/n$ we may apply the usual trick of averaging the projection~$M/n \to \langle m \rangle/n$ (with kernel~$L$) over the~$6$ elements of~$S_3$, and thus obtain an~$S_3$-equivariant projection~$p \colon M/n \to \langle m \rangle /n$. Put~$U= \ker p$, so~$M/n = \langle m \rangle/n \oplus U$ as~$S_3$-modules.

The kernel of~$M/n \to \bar M /n$ is~$\langle m \rangle /n$, so~$U$ is isomorphic to~$\bar M /n$. By lemma~\ref{lem-submods-of-Q} we see that~$\bar M$ is isomorphic to either~$Z$ or~$Q$, and thus by the last lemma~$U$ is isomorphic to~$Q/n$ in either case.

In the end we have proved that~$M/n \cong T/n \oplus Q/n \cong A/n$.
\end{proof}


We now use these lemma to study the groups~$G_n$ (for~$n$ prime to~$6$). Let us say that a subgroup~$H$ of~$G$ is {\em ample} if the induced map~$H \to S_3$ is surjective, and~$M = H \cap A$ has rank~$3$. Here and elsewhere we see~$A$ as~$\ker(G \to S_3)$. We will also say that~$(a, b) \in G\times G$ is an {\em ample pair} when~$\langle a, b \rangle$ is ample.

Let~$\left( (a_i, b_i) \right)_{i \in I}$ be the collection of all ample pairs. We let~$\widetilde G$ be the subgroup of the direct product
%
\[ \prod_{i \in I} \, \langle a_i, b_i \rangle  \]
%
generated by~$x= (a_1, a_2, \ldots )$ and~$y = (b_1, b_2, \ldots )$.

Consider the exact sequence
%
\[ 0 \longrightarrow \prod_{i \in I} M_i \longrightarrow \prod_{i \in
  I} \, \langle a_i, b_i \rangle \longrightarrow \prod_{i \in I} S_3 \longrightarrow 1 \, , \]
%
where~$M_i = \langle a_i, b_i \rangle \cap A$. It is easy to see that the images of~$x$ and~$y$ under the second map generate a group isomorphic to~$\bar S_3$, and in particular, finite. The kernel of~$\widetilde G \to \bar S_3$ will be written~$L$; as a subgroup of the finitely-generated group~$\widetilde G$ having finite index, we see that~$L$ is itself finitely generated, and it is abelian and torsion-free as a subgroup of~$\prod M_i$. Finally we see that~$L \cong \z^\omega $ for some number~$\omega $. [It is likely that, of all numbers, $\omega = 14$.] We note the exact sequence
%
\[ 0 \longrightarrow L \cong \z^\omega \longrightarrow \widetilde G
\longrightarrow \bar S_3 \longrightarrow 0 \, .  \]
%

Let~$H$ be an ample group. Then~$nM$ is characteristic in~$M$ and thus normal in~$H$, so there is a natural map~$H \to H/nM$. Combining these maps for different ample groups, we get a map
%
\[ \prod_{i \in I} \, \langle a_i, b_i \rangle \longrightarrow \prod_{i
  \in I} \, \langle a_i, b_i \rangle / nM_i \, .  \]
%

\begin{lem}
The images of~$x, y \in \widetilde G$ under this map generate a group isomorphic to~$\gb_n$ (with its canonical generators).
\end{lem}

\begin{proof}
Let~$H$ be ample. Since the order of~$M/nM$ is~$n^3$ which is prime to~$6$, the Schur-Zassenhaus theorem garantees that~$H / nM$ is a semi-direct product~$M/n \rtimes S_3$. For similar reasons, $G_n$ is a semi-direct product~$A/n \rtimes S_3$. By the above, $M/n \cong A/n$ as~$S_3$-modules, so there is an isomorphism of~$H/nM$ with~$G_n$.

Conversely, let~$a', b' \in G_n$ be such that~$\langle a', b' \rangle = G_n$. Pick~$a, b \in G$ mapping to~$a'$, $b'$ respectively under the natural map~$G \to G_n$. It is immediate that~$H = \langle a, b \rangle$ is ample, and~$H/nM \cong G_n$.

So the groups-with-distinguished-generators~$\langle a_i, b_i \rangle / nM_i$ are all isomorphic to~$G_n$ and represent each isomorphism class of pairs of generators for~$G_n$. The result follows.
\end{proof}

We have established the following.

\begin{prop}
When~$n$ divides~$m$, and~$m$ is prime to~$6$, we have maps
%
\[ \widetilde G \longrightarrow \gb_m \longrightarrow \gb_n
\longrightarrow \bar S_3 \]
%
compatible with the canonical generators. If we let~$K_n = \ker(\gb_n \to \bar S_3)$, then we have a surjective map~$L/n \to K_n$.  By Schur-Zassenhaus we have~$\bar G_n = K_n \rtimes \bar S_3$.

\end{prop}

[It is likely that the map~$L/n \to K_n$ is an isomorphism. GAP calculates that the kernel of~$\gb_n \to \bar S_3$ is~$\left(\z/n\right)^{14}$ for~$n=2, 3, 4, 5, 6, 7$; no counter-example yet.]



%% Here is a summary of the results of this section.

%% \begin{prop}
%% There is a group~$\widetilde G$, with distinguished generators~$x$
%% and~$y$, fitting in an exact sequence 
%% %
%% \[ 0 \longrightarrow L = \z^{14} \longrightarrow \widetilde G
%% \longrightarrow \bar S_3 \longrightarrow 0 \, .   \]
%% %
%% The subgroup~$nL$ is normal in~$\widetilde G$, and the factor group
%% is~$\gb_n$ when~$n$ is prime to~$6$. Thus there is an exact sequence
%% %
%% \[ 0 \longrightarrow \left(\z/n\right)^{14}  \longrightarrow \gb_n \longrightarrow \bar S_3 \longrightarrow 0 \, ,  \]
%% %
%% when~$gcd(n, 6)= 1$, and by Schur-Zassenhaus we have~$\gb_n =
%% \left(\z/n\right)^{14} \rtimes \bar S_3$.

%% All the homomorphisms in this proposition are compatible with the
%% canonical generators.
%% \end{prop}




\subsection{The group~$\bar S_3$}


In view of the above results, it is clear that~$\bar S_3$ will play an important role in the study of~$\bar G_n$, so we collect here some salient facts about this group. Everything can be obtained from GAP, so we will not give many details. The reader interested in checking everything ``by hand'' will start by proving that~$\bar S_3$ isomorphic to the subgroup of~$S_9$ (and in fact, of~$S_3 \times S_3 \times S_3$) generated by~$x_0 = (1, 2)(4, 5, 6)(8, 9)$ and~$y_0 = (1,3, 2)(4, 5)(7, 8)$. As a matter of notation, we think of~$S_3$ as~$G_0$, and so the map~$\gb \to \bar S_3$ will be written~$g \mapsto g_0$, and likewise for the various maps~$\gb_n \to \bar S_3$.

The order of~$\bar S_3$ is~$108 = 3^3 \cdot 2^2$, and in fact there is an exact sequence
%
\[ 1 \longrightarrow C_3^3 \longrightarrow \bar S_3 \longrightarrow
C_2^2 \longrightarrow 1 \, .  \]
%
The unique~$3$-Sylow is also the commutator subgroup. The generators~$x_0$ and~$y_0$ have order~$6$, and their centralizers are~$\langle x_0 \rangle$ and~$\langle y_0 \rangle$ respectively.

It is a fact that~$x_0^{-1}$ is conjugated to~$x_0$, and likewise for~$y_0$. Given that the group~$\bar S_3$ has exponent~$6$, it is standard to deduce:
%
\begin{lem} For any complex character~$\chi $ of~$\bar S_3$, we have~$\chi (x_0) \in \q$ and~$\chi(y_0) \in \q$.  \end{lem}

\begin{coro}
Assume~$n$ is prime to~$6$. For any complex character~$\chi$ of~$\gb_n$, the values~$\chi (x)$ and~$\chi (y)$ lie in~$\q(\mu_n)$, the field obtained by adjoining to~$\q$ the~$n$-th roots of unity.
\end{coro}

